Feedback Control of Turbulent Shear Flows by Genetic Programming

Turbulent shear flows have triggered fundamental research in nonlinear dynamics, like transition scenarios, pattern formation and dynamical modeling. In particular, the control of nonlinear dynamics is subject of research since decades. In this publication, actuated turbulent shear flows serve as test-bed for a nonlinear feedback control strategy which can optimize an arbitrary cost function in an automatic self-learning manner. This is facilitated by genetic programming providing an analytically treatable control law. Unlike control based on PID laws or neural networks, no structure of the control law needs to be specified in advance. The strategy is first applied to low-dimensional dynamical systems featuring aspects of turbulence and for which linear control methods fail. This includes stabilizing an unstable fixed point of a nonlinearly coupled oscillator model and maximizing mixing, i.e.\ the Lyapunov exponent, for forced Lorenz equations. For the first time, we demonstrate the applicability of genetic programming control to four shear flow experiments with strong nonlinearities and intrinsically noisy measurements. These experiments comprise mixing enhancement in a turbulent shear layer, the reduction of the recirculation zone behind a backward facing step, and the optimized reattachment of separating boundary layers. Genetic programming control has outperformed tested optimized state-of-the-art control and has even found novel actuation mechanisms.

==> s1.tex <==
\section{Introduction}

The control of turbulence is of fundamental importance 
for understanding of animal motion and 
for many engineering applications. 
It serves as one of the most complex paradigms 
for methods of the control of dynamical systems in general. 
%Due to the involved 
%bifurcation scenarios related to geometry, boundary conditions and parameters, 
%in particular 
%the Reynolds number, methods developed in the general context can be often 
%tested in a turbulent 
%situation. 
%\textcolor{red}{\bfseries [I do not understand this statement and suggest to delete the sentence].}
In fluid dynamics, many engineering applications benefit from feedback control, like 
drag reduction of transport vehicles
or green energy harvesting of wind and water 
flows.
In these fields, even small gain in energy savings are very important due to the 
huge 
number of vehicles, turbines, etc. involved. 
Apart from fluids, 
a generic control strategy for complex nonlinear systems
is desired in life sciences, 
medicine, and a vast number of engineering applications.

Apart from the importance of turbulence for applications, it serves as a paradigm for the study 
of complex dynamical systems. 
Fluid dynamics have led to many important discoveries and 
poses challenges to physics theory. 
Pattern formation, chaos and bifurcations, would not
have been found and studied without the driving force of turbulent flows.
So, we follow this line of thought and use turbulent flows as prototypic example
for a complex dynamical system. 
Yet, control strategies are best developed for simple nonlinear dynamical systems. 
Consequently, we study in this publication
the control of two systems with nonlinear features of turbulence:
(1) two coupled forced oscillators which are linearly uncontrollable, 
and (2) a forced Lorenz system,
where we optimize for mixing, i.e.\ aim at large Lyapunov exponents. 
Based on these results,
we apply our control algorithm to experiments with turbulence. 
%Let us introduce the problem of  control for flow systems:

For many laminar flows, linear control theory is used 
for the stabilization of a steady solution
by a local linearization of the Navier-Stokes equation.
Corresponding numerical and experimental stabilization studies include
virtually any configuration,
e.g. wakes ~\citep{Roussopoulos1993jfm},
cavity flows~\citep{Rowley2006arfm,sipp2007jfm,illingworth2012feedback},
flows of backward-facing step~\citep{Herve2012jfm},
boundary-layer flows~\citep{Bagheri2009jfm}.

Turbulent flows, however are next to impossible to stabilize, 
because of the huge number of degrees of freedom, 
the non-normal amplification mechanisms, 
complex bifurcations and nonlinear frequency cross talk.
In addition, real-world constraints complicate control, e.g. the cost of energy 
of actuators,
or their blank inability to control to a steady solution, because actuators 
cannot provide enough
energy or do not have the authority to force the fluid into a steady flow.
Linear control fails to handle frequency cross-talk between the coherent 
structures,
the mean flow and the stochastic small-scale fluctuations.
Yet, frequency cross-talk is an important actuation opportunity
as demonstrated by successful wake stabilization with
high-frequency 
actuation~\citep{Glezer2005aiaaj,thiria2006wake,Luchtenburg2009jfm}
and low-frequency forcing~\citep{Pastoor2008jfm}.
For real-world applications, model-based control of an experiment
requires a robust control-oriented reduced-order model
which is still a large challenge at this moment.
Such a reduced-order model needs --- at minimum ---
to resolve  the uncontrolled and controlled turbulent coherent structures
including the transients between them.

Intriguingly, animals have found feedback flow control solutions
neither knowing the Navier-Stokes equation nor reduced models thereof.
Examples are eagles whose feathers near the trailing edge move up to prevent stall.
Or dolphins whose compliant skins delay transition and thus decrease drag.
More than 50 years ago, Rechenberg \cite{Rechenberg1973book}
and Schwefel \cite{Schwefel1965diplom} 
have imitated nature's evolutionary principles
to solve engineering flow problems.
Subsequently, evolutionary algorithms have rapidly evolved
culminating in the genetic algorithm \cite{Holland1975book}
and genetic programming \cite{Koza1992}
and powerful methods of machine learning.
In the pioneering wall turbulence simulation of Lee et al. \cite{Lee1997},
a feedback law for skin friction reduction 
was learned in model-free manner employing a neural network.
The current study continues these works
and employs genetic programming as powerful regression technique
for the optimization of the multiple-input multiple-output control laws.

\begin{figure}
\begin{center}
\includegraphics[width=0.5\textwidth,natwidth=610,natheight=692]
{Control_class.pdf}
\end{center}
\caption{Decision tree for control design.}\label{fig:control_decision}
\end{figure}

In the following, we discuss in detail the different approaches on the example 
of turbulence. The paper is organized as follows:
In section~\ref{sec:GP}, we discuss the methodological approach; 
we present our novel model-free approach based on GP for 
controlling complex and turbulent flows.  We motivate the 
use of GP and describe the algorithm, called Genetic Programming Control (GPC). 
Then in section~\ref{sec:proof} we show the possibilities of GP-based model-free 
control by using it to stabilize a non-linear system exhibiting frequency 
cross-talk between two oscillators and to enhance the chaos in a periodic Lorenz 
system. In section~\ref{sec:exp} we display the successes obtained on 
experimental demonstrators including the mixing enhancement of a turbulent 
shear-layer, recirculation reduction on a backward facing step using real-time 
PIV and separation control on a separating turbulent boundary layer. 
Finally, we  discuss the advantages and drawbacks of the methods and conclude in 
section~\ref{sec:conclusion}. 


